Quantum Rational Transformation Using Linear Combinations of Hamiltonian Simulations

Rational functions are exceptionally powerful tools in scientific computing, yet their abilities to advance quantum algorithms remain largely untapped. In this paper, we introduce effective implementations of rational transformations of a target operator on quantum hardware. By leveraging suitable integral representations of the operator resolvent, we show that rational transformations can be performed efficiently with Hamiltonian simulations using a linear-combination-of-unitaries (LCU). We formulate two complementary LCU approaches, discrete-time and continuous-time LCU, each providing unique strategies to decomposing the exact integral representations of a resolvent. We consider quantum rational transformation for the ubiquitous task of approximating functions of a Hermitian operator, with particular emphasis on the elementary signum function. For illustration, we discuss its application to the ground and excited state problems. Combining rational transformations with observable dynamic mode decomposition (ODMD), our recently developed noise-resilient quantum eigensolver, we design a fully real-time approach for resolving many-body spectra. Our numerical demonstration on spin systems indicates that our real-time framework is compact and achieves accurate estimation of the low-lying energies.

==> IterativeFiltering.tex <==
\section{Iterative filtering for the ground and excited state problem}
\label{subsec:iterativeFiltering}

We now apply our real-time rational framework to address the problem of finding the low-energy states of a many-body Hamiltonian, a significant task encountered within physical, chemical, and materials sciences. 
Specifically, our goal is to construct an accurate rational approximation of the step function, or equivalently the signum function, as a spectral filter.

Let $H = \sum_{n=0}^{N-1} E_n \ket{E_n} \bra{E_n}$ be the eigen-decomposition of the Hamiltonian, where we order the eigenvalues $E_0 \leq E_1 \leq \cdots \leq E_{N-1}$ in a nondecreasing order. Observe that a step function $\Theta(\omega - E)$ filters out the components of any initial state with energies above $E$, \textit{i.e.},
\begin{align}
    \Theta(H - E) = \sum_{n=0}^{N_{c}} \ket{E_n} \bra{E_n},
\end{align}
where $N_c$ denotes a threshold eigenindex satisfying $E_{N_{c}} < E < E_{N_{c} + 1}$.
Therefore, 
setting $E = E_{\rm threshold}$ to the relevant threshold energy, 
we selectively annihilate all but a low-energy subspace of the full Hilbert space. Within this invariant subspace of size $\mathcal{O}(1)$, we can then efficiently resolve the energies of interest. 
% Therefore, setting $E = E_0 + \mathcal{O} ( \frac{1}{N} )$, we selectively annihilate all but a low-energy subspace of the full Hilbert space. Within this invariant subspace of size $\mathcal{O}(1)$, we can resolve the energies of interest. 



Instead of relying on an idealized step filter, in practice we seek a rational approximant $r_{E}(\omega)$ of $\Theta(\omega-E)$ so that,
\begin{align}
    \lvert r_{E}(E_n) \rvert \approx \begin{cases}
    1 & {\rm if}~ E_n \leq E - \Delta E,  \\
    0 & {\rm if}~ E_n \geq E + \Delta E,
    \end{cases}
\end{align}
where $\Delta E$ characterizes the width of buffer region over which the value of $\lvert r_E \rvert$ transitions roughly from $1$ to $0$. Let us fix $\Delta E$. Additionally, we suppose knowledge of the spectral bounds, $E_{-} \leq E_n \leq E_{+}$, where the precise largest and smallest eigenenergies do not need to be known in advance. 
%A filtering procedure relying on the rational filter $r_E(H)$ reduces the effective spectral range by a factor of $\xi = \frac{E + \Delta E - E_{-}}{E_{+} - E_{-}}$ upon suitable choices of $E$ and $\Delta E$.
%% Setting $\Delta E = \mathcal{O}(\frac{1}{N})$ for a rational filter, unlike the perfect step filter, proves ineffective since the approximation error cannot be controlled even with an optimal approximant $r_K$ exhibiting exponential convergence. Recall the sharp error $e^{- \pi^2 K/2\mu(\Delta E)}$ (c.f. \cref{eq:sign_bound}) of a Zolotarev approximant: the term $\mu(\frac{{\rm constant}}{N})$ would grow exponentially with the system size, necessitating an exponentially higher rational degree. Let us thus fix $\Delta E$ to be a constant.
%To refine the filtering procedure and achieve a reduction of the spectral range $[E_{-}, E_{+}] \mapsto [E_{-}, E_{-} + \delta E]$ for arbitrary $\delta E$, we consider a linear transformation
%\begin{align}
    %f_{\xi}(H) = \frac{1}{\xi}(H- E_{-}) + E_{-}, \\
    %... (r_E \circ f_{\xi^3}) (r_E \circ f_{\xi^2})(r_E \circ %f_{\xi})r_{E},
%\end{align}
%where we simply scale and shift the Hamiltonian. 

The Zolotarev rational function and the rational function obtained by the least-squares approach can be used to determine poles so that the step function is approximated up to a desired accuracy.
Alternatively, a fixed rational function achieving a lower approximation accuracy can be applied iteratively and also obtain accurate eigenenergy approximations.
We will argue that, since the cost of resolvent simulation is determined by the distance $b_k$ of the pole $z_k=a_k+b_k i$ to the real line and by the distance of $a_k$ to the spectrum of the (filtered) Hamiltonian of interest, each iteration can be performed at a constant cost.

In order to achieve a reduction of the spectral range $[E_{-}, E_{+}] \mapsto [E_{-}, E_{-} + \delta E]$ for arbitrary $\delta E$, we propose a repeated application of a fixed rational filter $r_E$ to the matrix alternated by a shift and rescale of the resulting matrix using $f_\xi$.
That is, applying $r_E(H)$ supresses the eigenvalues in the interval $[E+\Delta E,E_+]$, thereby reducing the effective spectral range by a factor $\xi = \frac{E + \Delta E - E_{-}}{E_{+} - E_{-}}$.
The linear transformation $f_{\xi}(r_E(H)) = \frac{1}{\xi}(H- E_{-}) + E_{-}$ rescales the spectrum of the matrix $r_E(H)$ such that it is again approximately $[E_-,E_+]$, allowing for the same filter $r_E$ to be applied again.
For a given $\delta E$, this process can be repeated $n = \mathcal{O}(\log_{\xi} \delta E)$ times,
\begin{equation}
    (r_E \circ f_{\xi^n})... (r_E \circ f_{\xi^3}) (r_E \circ f_{\xi^2})(r_E \circ f_{\xi})r_{E},
\end{equation}
which reduces the effective spectral range to $[E_-,E_-+\delta E]$, where we can choose $\delta E$ such that $E_-+\delta E = E_{\rm threshold}$.
The application of this process to filter out high energy eigenstates from some given initial state is illustrated in \cref{fig:iterativeFiltering}. 
This figure shows the process for the step function $\Theta(\omega-0.5)$, in practice a rational filter $r_E(H)$ that approximates the step function is employed.


\begin{figure}[!ht]
    \centering
    \setlength\figureheight{1.7cm}
    \setlength\figurewidth{0.3\textwidth}	
    \begin{subfigure}[t]{0.33\textwidth}
        \input{figs/iterativeFiltering_11.tikz}    
        \caption{Effective spectrum of $H$ with respect to initial state $\vert \phi\rangle$. Rescaled using spectral bounds $E_-$ and $E_+$ of $H$.}
    \end{subfigure}
    \begin{subfigure}[t]{0.32\textwidth}
        \input{figs/iterativeFiltering_12.tikz}    
        \caption{Effective spectrum of the rescaled $f_{\xi}(H)$ with respect to the filtered state $\Theta(H-0.5) \vert \phi\rangle$.}
    \end{subfigure}
    \begin{subfigure}[t]{0.32\textwidth}
        \input{figs/iterativeFiltering_13.tikz}    
        \caption{Effective spectrum of $f_{\xi^2}(H)$ with respect to the filtered state $\Theta(H-0.5) f_{\xi}(H)\Theta(H-0.5)\vert \phi\rangle$.}
    \end{subfigure}

    \begin{subfigure}[t]{0.32\textwidth}
        \input{figs/iterativeFiltering_21.tikz}    
        \caption{Construct filter $\Theta(H-0.5)$ shown by dashed line.}
    \end{subfigure}
    \begin{subfigure}[t]{0.32\textwidth}
        \input{figs/iterativeFiltering_22.tikz}    
        \caption{Reuse filter $\Theta(H-0.5)$.}
    \end{subfigure}
    \begin{subfigure}[t]{0.32\textwidth}
        \input{figs/iterativeFiltering_23.tikz}    
        \caption{Reuse filter $\Theta(H-0.5)$.}
    \end{subfigure}

    
    \begin{subfigure}[t]{0.32\textwidth}
        \input{figs/iterativeFiltering_31.tikz}    
        \caption{Applying filter $\Theta(H-0.5)\vert \phi\rangle$ suppresses high energy eigenenstates in $\vert \phi\rangle$.}
    \end{subfigure}
    \begin{subfigure}[t]{0.32\textwidth}
        \input{figs/iterativeFiltering_32.tikz}    
        \caption{More high energy eigenstates are suppressed by filtering again $\Theta(H-0.5) f_{\xi}(H)\Theta(H-0.5)\vert \phi\rangle$.}
    \end{subfigure}
    \begin{subfigure}[t]{0.32\textwidth}
        \input{figs/iterativeFiltering_33.tikz}    
        \caption{The third filtering suppresses all eigenstates with positive eigenenergy in the state.}
    \end{subfigure}
    \caption{In the procedure of recursive filtering the goal is to suppress high energy eigenstates in some initial state $\vert \phi\rangle$. 
    The eigenenergies corresponding to eigenstates that appear in a (filtered) state are shown as $({\color{blue}\ast})$, i.e., the effective spectrum.
    Let us suppress all eigenstates belonging to nonnegative eigenenergies, as shown in the left upper figure.
    The filtering is a repetition of three steps.
    First, a shift and rescale of the effective spectrum to $[-1,1]$ is performed.
    Second, a filter, e.g., $\Theta(\omega-0.5)$, is constructed that removes eigenstates corresponding to high eigenenergies, the filter is shown with a dashed line.
    The repeated shifting and rescaling of the effective spectrum by $f_\xi^n$ allows us to reuse the same filter $\Theta(\omega-0.5)$.
    Third, the filter is applied to the state, resulting in a smaller effective spectrum of $H$.}
    \label{fig:iterativeFiltering}
\end{figure}


%Observe that the product of the rational functions $(r_{E} \circ f_{\xi}) r_{E}$ preserves eigenenergies only in the range $[E_{-}, E_{-} + \xi^2(E_{+} - E_{-})]$. Consequently, repeated applications of the transformed rational filters can compress the spectral range to a desired accuracy $\delta E$ in $\mathcal{O}(\log_{\xi} \delta E)$ iterations. 
Given the form of a rational filter $r_E (H) = \sum_{k=0}^{K-1} c_{k} R(z_{k}) + {\rm h.c.}$ (where ${\rm h.c.}$ denotes Hermitian conjugate), we have,
% $r_E \circ f_{\xi} \circ \cdots r_E \circ f_{\xi}$
\begin{align}
    (r_E \circ f_{\xi})(H) = \sum_{k=0}^{K-1} \xi c_{k} R( f_{1/\xi}(z_{k}) ) + {\rm h.c.},
\end{align}
where the resolvent identity \cite{Yo95} implies,
\begin{align}
   [(r_{E} \circ f_{\xi}) r_E] (H) &= \sum_{k,k'=0}^{K-1} \sum_{\iota, \iota' = \pm} \xi c_{k \iota} c_{k' \iota'}  R( f_{1/\xi}(z_{k \iota}) ) R(z_{k' \iota'}), 
   \label{eq:resolvent_product}\\
   &= \sum_{k,k'=0}^{K-1} \sum_{\iota , \iota' = \pm} \frac{\xi c_{k \iota} c_{k' \iota'}}{\tilde{z}_{k' \iota'} - \xi \tilde{z}_{k \iota} } \left[  R( f_{1/\xi}(z_{k \iota}) ) -  R(z_{k' \iota'}) \right] ,
\end{align}
with $c_{k\pm} = \Re c_k \pm i \Im c_k$, $z_{k\pm} = a_k \pm i b_k$, and $\tilde{z}_{k \pm} = z_{k \pm} - E_{-}$. For simplicity, we introduce the subscript $\iota$ to designate the complex conjugation of a scalar or the Hermitian conjugation of an operator. The action of the composed filter $r_{\star 1}(H;\xi) = [(r_{E} \circ f_{\xi}) r_E ] (H)$ on any initial state $\ket{\phi}$ can be computed as
\begin{align}
    \begin{split}
        \braket{\phi| f(H) r_{\star 1}(H;\xi) |\phi} = \xi \sum_{k=0}^{K-1} \sum_{\iota = \pm} & c_{k\iota}^{(1)}(\xi) \braket{\phi|f_{\iota}(H) R( f_{1/\xi}(z_{k}) )|\phi}_{\iota} \\
        &+ \sum_{k=0}^{K-1} \sum_{\iota = \pm} c^{(1)}_{k\iota}(1/\xi) \braket{\phi|f_{\iota}(H) R(z_{k})|\phi}_{\iota},
    \end{split}
    % &= \sum_{k,k'=0}^{K-1} \sum_{\iota, \iota' = \pm}  \frac{\xi c_{k \iota} c_{k' \iota'}}{\tilde{z}_{k' \iota'} - \xi \tilde{z}_{k \iota} } \left[ \braket{\phi|R( f_{1/\xi}(z_{k}) )|\phi}_{\iota} -  \braket{\phi|R(z_{k'})|\phi}_{\iota'} \right],
\end{align}
where, 
\begin{align}
    c_{k\iota}^{(1)}(\xi) = \sum_{k'=0}^{K-1} \sum_{\iota'=\pm} \frac{ c_{k \iota} c_{k' \iota'} }{\tilde{z}_{k' \iota'} - \xi \tilde{z}_{k \iota} }.
\end{align}
That is, we have converted the evaluation of $K^2$ resolvent products (c.f. \cref{eq:resolvent_product}) to that of $2K$ resolvents within a single iterative filtering step. Therefore, applying the resolvent identity recursively, we can implement the filter after $D$ iterations,
\begin{align}
   r_{\star D} (H;\xi) = \prod_{d=0}^{D} r_{E} \circ f_{\xi^{d}} (H), 
\end{align}
via evaluation of $(D+1)K$ resolvents (rather than that of $K^{D+1}$ resolvent products). For a wide variety of many-body Hamiltonians $H$, the low-energy sector of the spectrum $\delta E$ is $\mathcal{O} (\frac{1}{{\rm polylog}N} )$ relative to the spectral range. This results in $D = \log_{1/\xi} {\rm polylog} N$ iterations, where the cost of the filtering procedure is determined by the pole locations $\frac{b_k}{{\rm polylog}N}$ (the imaginary parts are scaled towards zero by a factor of $\xi$ with each iteration).


As a concrete example, let us consider the Zolotarev approximant, $r_{E}(H) = \frac{1 - r_{K}(H)}{2}$, and a discrete-time scheme for constructing the iterative filter $r_{\star D}(H)$. In order to evaluate the expectations in \cref{eq:filtered_obs}, we need to run time evolutions of the form $e^{-iH(\tau_i+t_j)}$, where $\tau_i$ advances the observable vectors $o_{\star}$ and $t_j$ compiles the rational filter $r_{\star D}$. Let us denote the sequence of distinct evolution times by $\bt_{\star}$. First observe that 
\begin{align}
    r_{\star D}(H;\xi) = \frac{1}{2^{D+1}} \sum_{d=0}^{D+1} (-1)^d \sum_{\bs \subseteq [D]: \lvert \bs \rvert = d} \prod_{i=0}^{d-1} r_{K} \circ f_{\xi^{s_i}} (H),
\end{align}
where each $\bs = [s_0, s_1, \cdots, s_{d -1}]$ is a multi-index specified by distinct $s_i \in [D]$. We simply assume that $\bs$ is ordered with $s_i < s_{i+1}$. Thus to construct a discrete-time filter $\epsilon$-close to $r_{\star D}(H)$, it suffices to adopt a Legendre rule $\bt$ such that
\begin{align}
    \bigg\lVert \prod_{i=0}^{d-1} r_{K} \circ f_{\xi^{s_i}}(H) - \sum_{j=0}^{J-1} x_j e^{-iHt_j} \bigg\rVert_2 \leq \epsilon,
\end{align}
for all multi-indices $\bs$. We assert that $[D]$ incurs the largest error among the multi-indices since by \cref{cor:1},
\begin{align}
    J_{\bs} = \log_{2} \log \frac{ 2 (\gamma_K)^{d} \lVert \bc_{\bs} \rVert_1 }{ \epsilon \xi^{\lVert \bs \rVert_{\infty} } b^{-} } +   \frac{3b^{-} + 2\sqrt{2} b^{-}  + \lVert H \rVert_2}{4\sqrt{2} b^{-}} \log_2 \frac{ 2 (\gamma_K)^{d} \lVert \bc_{\bs} \rVert_1}{ \epsilon \xi^{\lVert \bs \rVert_{\infty}} b^{-} } +3,
\end{align}
and 
\begin{align}
    \lVert \bt_{\bs} \rVert_{\infty} = \frac{1}{ \xi^{\lVert \bs \rVert_{\infty}} b^{-}} \log \frac{ (\gamma_K)^{d} \lVert \bc_{\bs} \rVert_1 }{ \epsilon \xi^{\lVert \bs \rVert_{\infty}} b^{-}},
\end{align}
where $\bc_{\bs}$ is the vector of rational coefficients satisfying
\begin{align}
    \prod_{i=0}^{d-1} r_{K} \circ f_{\xi^{s_i}}(H) = (-\gamma_K)^{d} \sum_{i=0}^{d-1} \sum_{k=0}^{K-1} \sum_{\iota = \pm}  (c_{\bs})_{i k \iota}  R ( f_{1/\xi^{s_i}}(z_{k\iota}) ),
\end{align}
with $\lVert \bc_{\bs} \rVert_1$ bounded by $\xi^{\lVert \bs \rVert_{\infty}}$.  We note that the spectral transformation $H \mapsto f_{\xi}(H)$ does not stretch the effective Hamiltonian spectral range, since we apply the transformed filters in a sequential way. For example application of the initial filter $r_K(H)$ almost `eliminates' the components of the state $\ket{\phi}$ in the energy range $[E+\Delta E, E_{+}]$, which also holds during succeeding iterative steps that operate on a smaller and smaller effective spectral range.



%%%%%% [YS:] I would keep the ODMD stuff in the same subsection %%%%%%

% \subsection{Application to the ground and excited state problem}
% \label{subsec:application}
% We now apply our real-time rational framework to address the problem of finding the low-energy states of a many-body Hamiltonian, a significant task encountered within physical, chemical, and materials sciences. 


%The construction of such an iterative filter can be integrated as a pre-processing routine for a suitable quantum eigensolver. In particular, we illustrate how to combine the filtering technique with our recently developed real-time approach for eigenenergy estimation. We focus on the observable dynamical mode decomposition (ODMD)~\cite{shen2023estimating} that measures the real-time expectations,
%\begin{align}
%	o(\tau_j) =  \braket{\phi| e^{-iH \tau_j } |\phi} = \sum_{n=0}^{N-1} p_n e^{-iE_n \tau_j}, \qquad \tau_j = j \Delta \tau,
%	\label{eq:odmd}
%\end{align}
%on the quantum computer. ODMD is based on the classical dynamic mode decomposition (DMD) method, which linearizes the time evolution of state vectors by solving an efficient least-squares problem. In ODMD, the state vectors are not the quantum states themselves but rather the time-delayed `observable vectors', $[o(\tau_j), o(\tau_{j+1}), \cdots, o(\tau_{j+Q-1 })]$, for some delay period $Q$. The expectations collected from successive time evolutions with a timestep $\Delta \tau$ allows us to identify a least-squares solution $B$ satisfying,
%\begin{align}
%	\begin{bmatrix}  
%		o(\tau_1) & o(\tau_2) & o(\tau_3) & \cdots \\
%		o(\tau_2) &  o(\tau_3) &  o(\tau_4) & \cdots \\
%		o(\tau_3) &  o(\tau_4) &  o(\tau_5) & \cdots \\
%		\vdots & \vdots & \vdots & \ddots
%	\end{bmatrix} \stackrel{{\rm LS}}{=} B \begin{bmatrix}  
%		o(\tau_0) & o(\tau_1) & o(\tau_2) & \cdots \\
%		o(\tau_1) &  o(\tau_2) &  o(\tau_3) & \cdots \\
%		o(\tau_2) &  o(\tau_3) &  o(\tau_4) & \cdots \\
%		\vdots & \vdots & \vdots & \ddots
%	\end{bmatrix},
%	\label{eq:odmd_LS}
%\end{align}
%where $B$ is the so-called system matrix that contains the key frequency/energy information for advancing each observable vector a timestep $\Delta \tau$ forward. We sample over a relatively small number of timesteps so that $B$, upon a regularization, remains
%well-conditioned and compact in size. This makes its classical diagonalization viable: the extremal eigenphase, $\Tilde{E}_0 = \frac{1}{\Delta \tau} \max_{\lambda_{B}} {\rm arg}(\lambda_{B})$ for eigenvalues $\lambda_{B}$ of $B$, provides a robust and reliable estimate of the exact ground state energy $E_0$.
%
%From the signal processing perspective, we observe that \cref{eq:odmd} can be understood as sinusoidal data comprised of exponentially many components $e^{-iE_n \tau_j}$, each oscillating in time at its own frequency. To remove the high-energy components, we consider measuring the filtered expectations,
%\begin{align}
%	o_{\star}(\tau_j) = \braket{\phi| e^{-iH \tau_j }  r_{\star D}(H;\xi) |\phi} \approx \sum_{n = 0}^{N_{c}} p_n e^{-iE_n \tau_j},
%	\label{eq:filtered_obs}
%\end{align}
%where $N_{c}$ is an eigenindex such that $E_{N_c} \lesssim E_{-} + \delta E \lesssim E_{N_c + 1}$. The filtered expectations $o_{\star}$ can be computed with a sequence of time-evolution circuits as discussed in \cref{subsec:Zolotarev_approx,subsec:LS_approx}. Following the filtering procedure, we find a new system matrix $B_{\star}$ that effectively describes the dynamics within some low-energy subspace. Diagonalization of $B_{\star}$ thereby enables a simultaneous estimation of eigenenergies in this subspace.
%
%The total simulation cost for computing the filtered expectations is bounded by $\lVert \bt_{\star} \rVert_{1} = J_{\bs} N_c \left[ (N_{c}-1) \Delta \tau + \lVert \bt_{\bs} \rVert_{\infty} \right]$ for $\bs = [D]$.  % {\color{red}[NVB: What is $N_c$?]} \textcolor{blue}{[$N_c$ is defined below Eq. (75) -- it is the number of eigenvalues we want to estimate which is typically of $\mathcal{O}(1)$ since we only want a few of them]}. 
%That is, by choosing the Zolotarev degree $K$ and Hamiltonian spectral parameters $(E_{\pm}, \Delta E)$, we are able to achieve the Heisenberg-limited scaling $\lVert \bt_{\star} \rVert_1 = \Tilde{O}(\frac{1}{\delta E})$.


==> Quadrature.tex <==

\section{Efficient computation of the resolvent}
%\label{sec:resolvent}
In order to use a rational filter in eigenvalue computation, we have to compute the resolvents $v^\ast (z-H)^{-1} v$ efficiently on quantum hardware.
Resolvents also occur in the quantum linear system problem \cite{HHL} and in Green's function \cite{something}.

The resolvent can be written in terms of an integral of matrix exponentials, depending on the shift $z$ we distinguish three expressions:
\begin{align}
    (z - H)^{-1} &= -i \int_{0}^{\infty} dt~ e^{i(z-H)t}  \text{ when } |\Im{z}| > 0. \label{eq:single}\\
    (z - H)^{-1} &= \frac{i}{\sqrt{2\pi}} \int_{0}^{\infty} dy \int_{-\infty}^{\infty} dt~ t e^{-t^2/2} e^{iy(z-H)t} \text{ when } \Im{z} = 0,\label{eq:double2}\\
    (z - H)^{-1} &= \mp \frac{1}{\pi} \int_{0}^{\infty} dy \int_{-\infty}^{\infty} dt~ e^{-t^2/2} e^{iy(z-H)t} \text{ when } \Im{z} = 0 \text{ and } \Re{z} \notin [E_0, E_{N-1}], \label{eq:double2}
\end{align}


\subsection{Quadrature rules}
A quadrature rule provides an approximation to an integral in the form of a weighted sum of function evaluations,
\begin{equation*}
    \int_{a}^b dt~ f(t) \approx \sum_{k=1}^K w_k f(t_k),
\end{equation*}
where $\{t_k\}_{k=1}^K$ are the called nodes and $\{w_k\}_{k=1}^K$ the weights.
For the integral expressions of the resolvent, discretization via a quadrature rule results in a sum of matrix exponentials $e^{i(z-H)t_k}$, quantities that can be computed efficiently on quantum hardware in the form $v^\ast e^{i(z-H)t_k} v$.
In the sequel we discuss quadrature rules for the three expressions \eqref{eq:single}-\eqref{eq:double2}.

\subsubsection{Single integral formulation}
For the single integral formulation
\begin{equation*}
    (z - H)^{-1} = -i \int_{0}^{\infty} dt~ e^{i(z-H)t}  \text{ when } |\Im{z}| > 0,
\end{equation*}
a quadrature on the half real line is suitable.
The Gauss-Laguerre quadrature rule $\{t^{\rm La}_k,w^{\rm La}_k\}_{k=1}^K$ takes as nodes the zeros of the Laguerre polynomials and weights such that the approximation is exact for integrating polynomials up to degree $2K-1$.
The corresponding approximation is
\begin{equation*}
    -i \int_{0}^{\infty} dt~ e^{-t} e^{i((z+1)-H)t} \approx -i \sum_{k=1}^K w^{\rm La}_k e^{i((z+1)-H)t_k^{\rm La}},
\end{equation*}
and has, {\color{red}under certain conditions on its Taylor coefficients}, geometric rate of convergence \cite{Lu83}.

Since the integrand decays exponentially at the rate $e^{-\Im(z)t}$, it is possible to truncate the infinite interval $[0,\infty]$ to a finite interval $[0,T]$, where $T = \frac{-\log(\epsilon)}{\Im(z)}$ for some small $\epsilon>0$.
Note that if $\Im(z)<0$, we can use the identity $(z-H)^{-\ast} = (\Bar{z}-H)^{-1}$ to get a decaying integrand.
The truncation of the interval results in a truncation error
\begin{equation*}
	\left\Vert \int_{0}^{\infty} dt~ e^{i(z-H)t}  - \int_{0}^{T} dt~ e^{i(z-H)t} \right\Vert_\infty  = \mathcal{O}(\epsilon).
  \end{equation*}
After truncation, we can employ the trapezoidal rule to discretize the integral, 
\begin{equation*}
    -i \int_{0}^{\infty} dt~ e^{-t} e^{i(z-H)t} \approx -i \sum_{k=1}^K  w_k^{\rm trap} e^{i(z-H)t_k^{\rm trap}},
\end{equation*}
which uses equidistant nodes $t_k^{\rm trap} = (k-1)h$, with step size $h = T/(K-1)$, and weights $w_1^{\rm trap} = w_K^{\rm trap}= h/2$, and $w_k^{\rm trap} = h$, for $k=2,\dots,K-1$.
In general, the trapezoidal rule converges with second order of the step size, i.e., $\mathcal{O}(h^{-2})$.

A faster converging approximation can be obtained by employing the Gauss-Legendre quadrature rule, which uses the zeros of the $K$-degree Legendre polynomials as nodes $\{t_k^{\rm Leg}\}_{k=1}^K$.
The corresponding weights $\{w_k^{\rm Leg}\}_{k=1}^K$ are taken such that this rule integrates polynomials up to degree $2K-1$ exactly.
Since Legendre polynomials have zeros in the interval $[-1,1]$, we will rescale the integral before using the quadrature rule
\begin{equation*}
    -i \int_{0}^{\infty} dt~ e^{-t} e^{i(z-H)t} = -i \frac{T}{2}  \int_{-1}^1 dt~  e^{i \frac{T}{2}(z-H)(t+1)} 
    \approx -i \frac{T}{2} \sum_{k=1}^K w_k^{\rm Leg} e^{i \frac{T}{2}(z-H)(t_k^{\rm Leg}+1)}.
\end{equation*}

From \cite{vS77} we know that the Gauss-Legendre quadrature error for a function $f(x)$ that is analytic in and on the ellipse $\mathcal{E}_\rho:=\{z\in\mathbb{C}\vert z= \frac{1}{2} (u+u^{-1}), u = \rho e^{i\theta}, -\pi \leq \theta \leq \pi\}$ is 
\begin{equation}\label{eq:GaussLegendre_bound}
	\vert \mathcal{I}-\mathcal{I}_K\vert  \leq \frac{8M}{\rho^{2K} (1-\rho^{-2})},
\end{equation}
where $M:= \max_{x\in \mathcal{E}_\rho} \vert f(x)\vert$.
Since the integrand is an entire function, this bound holds for every $\rho>1$, however, note that the right hand side is not monotonically decreasing as $\rho$ increases due to the dependence of $M$ on $\rho$.

\subsubsection{Double integral formulation}
For $z\notin [E_0,E_{m-1}]$, the integral expression is given by the double integral
\begin{equation}\label{doubleIntegral_out}
    (z-H)^{-1} = \mp \frac{1}{\pi} \int_{0}^{\infty} dy \int_{-\infty}^{\infty} dt~ e^{-t^2/2} e^{iy(z-H)t}.
\end{equation}
Since any quadrature rule, with nodes $\{t_n\}_{n=-N}^N$ and weights $\{\alpha_n\}_{n=-N}^N$, for the inner integral results in	
\begin{equation*}
    \frac{i}{\sqrt{2\pi}} \int_{0}^{\infty} dy \int_{-\infty}^{\infty} dt~ t e^{-t^2/2} e^{iy(z-H)t} \approx \frac{i}{\sqrt{2\pi}}  \sum_{n=-N}^N \alpha_n t_n e^{-t_n^2/2} \int_{0}^{\infty} dy~ e^{iy(z-H)t_n},
\end{equation*}
which is a sum of single integrals of the form discussed above.
The truncation of the integration interval at $Y := \frac{\sqrt{-2\log(\epsilon)}}{\Delta}$, with $\Delta:=\min(\vert z-E_0 \vert,\vert z-E_{m-1} \vert)$, results in an error 
\begin{equation*}
    \left\vert \int_{0}^{\infty} dy~ e^{iy(z-H)t_n} - \int_{0}^{Y} dy~ e^{iy(z-H)t_n} \right\vert = \mathcal{O}(\epsilon).
\end{equation*}
{\color{red} TODO: add proof here or in appendix}

Next, we focus on the quadrature rules for the inner integral
\begin{equation*}
    \int_{-\infty}^\infty dt~ e^{-t^2/2} e^{iy(z-H)t}.
\end{equation*}
The Gauss-Hermite quadrature rule $\{t_\ell^{\rm He},w_\ell^{\rm He}\}$ uses zeros of the Hermite polynomials as nodes and can be applied after setting $\tau=t/\sqrt{2}$,
\begin{equation*}
    %\sqrt{2} \int_{-\infty}^\infty dt~ e^{-\tau^2} e^{iy(z-H)\tau/\sqrt{2}} 
    \int_{-\infty}^\infty dt~ e^{-t^2/2} e^{iy(z-H)t}
    \approx \sqrt{2} \sum_{\ell=1}^L w_\ell^{\rm He}  e^{iy(z-H)t_\ell^{\rm He}/\sqrt{2}}.
\end{equation*}
Alternatively, the interval $[-\infty,\infty]$ can be truncated to a finite interval $[-S,S]$.
The truncation at $S=\sqrt{-2\log \epsilon}$ results in a truncation error
\begin{equation*}
    \left\vert \int_{-\infty}^\infty dt~ e^{-t^2/2} e^{iy(z-H)t} - \int_{-S}^S dt~ e^{-t^2/2} e^{iy(z-H)t} \right\vert = \mathcal{O}(\epsilon).
\end{equation*}
Moreover, since we have for some small $\delta>0$ that $\vert f(S+\delta)-f(-S-\delta)\vert< \epsilon$, the integrand is periodic up to precision $\epsilon$.
Thanks to this (finite precision) periodicity of the integrand, the trapezoidal rule on $[-S,S]$ converges exponentially \cite{TrWe14}.
That is, for an even number $L$, the nodes are $t_\ell^{\rm trap} = (\ell-L/2) h$ , with step size $h = 2 S/L$ and $\ell=0,1,\dots, L$. 
The approximation is
\begin{equation*}
    \int_{-\infty}^\infty dt~ e^{-t^2/2} e^{iy(z-H)t} \approx \int_{-S}^S dt~ e^{-t^2/2} e^{iy(z-H)t} \approx h \sum_{\ell=0}^L e^{-\ell^2 h^2/2} e^{iyh(z-H)\ell}.
\end{equation*}
This approximation converges exponentially, i.e., at a rate $\mathcal{O}(e^{-L})$, up to relative precision $\mathcal{O}(\epsilon)$.

For the finite interval $t\in[-S,S]$, we can also use Gauss-Legendre rule $\{t_{\ell}^{\rm Leg},w_{\ell}^{\rm Leg}\}_{\ell=1}^L$ after rescaling the interval to $\tau\in[-1,1]$,
\begin{equation*}
    \int_{-S}^S dt~ e^{-t^2/2} e^{iy(z-H)t} =  S \int_{-1}^1 d\tau~ e^{-S^2 \tau^2/2} e^{iSy(z-H)\tau} \approx \sum_{\ell=1}^L w_{\ell}^{\rm Leg} e^{-S^2 (t_{\ell}^{\rm Leg})^2/2} e^{iSy(z-H)t_{\ell}^{\rm Leg}}.
\end{equation*}
The convergence rate is given by \eqref{eq:GaussLegendre_bound}.

{\color{red} TODO: add comments on other double integral. For trunction, use $Y/10$, which is not optimal but easy to compute.}


\subsection{Cost analysis}
Thanks to the quadrature rules, the resolvent $(z-H)^{-1}$ can be approximated by a weighted sum of matrix exponentials $e^{-iHt}$ at different times $t$.
A larger $t$ requires a longer simulation time, which makes it more expensive {\color{red} TODO: some reference here}.
We discuss metrics that quantify the cost of simulation in terms of time and perform numerical experiments to identify the most efficient quadrature rule.

\subsubsection{Metrics for time evolution}
For a quadrature rule with nodes $\{t_k\}_{k=1}^K$ for the single integral, the relevant metrics are $t_{\rm max} = \underset{k}{\max}~t_k $ and $t_{\rm tot} = \sum_{k=1}^K t_k$.
These metrics are shown in Table \ref{table:cost_evolutionTime} for the three quadrature rules discussed above.
\begin{table}[!ht]
	\centering
	\begin{tabular}{l|ll}
		Single integral & $t_{\rm max}$  & $t_{\rm tot}$  \\ \hline
		Gauss-Legendre & $T=-\log(\epsilon)/b$            & $TK/2$ \\
		Trapezoidal    & $T=-\log(\epsilon)/b$            & $TK/2$ \\
		Gauss-Laguerre & $\approx 4K+2$ & $K^2$         
	\end{tabular}
	\caption{Table summarizing the time metrics for the quadrature rules with $K$ nodes for discretizing the single integral. For the Gauss-Legendre and trapezoidal rule, the interval $[0,T]$ is used.}
	\label{table:cost_evolutionTime}
\end{table}

For quadrature rules for a double integral, with nodes $\{y_k\}$ for outer and $\{t_\ell\}$ for the inner integral, the metrics are $t_{\rm max} = \underset{k,l}{\max}~ y_k\vert t_\ell\vert $ and $t_{\rm tot} = \sum_{k,l} y_k\vert t_\ell\vert$. 
In Table \ref{table:cost_evolutionTime_double} we show the time metrics for the quadrature rules applied to the double integral, where the outer integral is discretized using the Gauss-Legendre rule on $[0,Y]$, with $Y = \frac{\sqrt{-2\log(\epsilon)}}{\Delta}$.
\begin{table}[!ht]
	\centering
	\begin{tabular}{l|ll}
		Double integral & $t_{\rm max}$  & $t_{\rm tot}$  \\ \hline
		Gauss-Legendre & $YS$            & $??$ \\
		Trapezoidal    & $YS$            & $\frac{YKS(L+2)}{4}$ \\
		Gauss-Hermite & $??$ & $??$         
	\end{tabular}
	\caption{Table summarizing the time metrics for the quadrature rules with $K$ nodes for discretizing the double integral. 
    The outer integral is discretized with a Gauss-Legendre rule on $[0,Y]$.
    The corresponding metrics for the Gauss-Legendre and trapezoidal rule on the interval $[-S,S]$, and Gauss-Hermite are shown.}
	\label{table:cost_evolutionTime_double}
\end{table}

\subsubsection{Numerical experiments -- single integral}
First, we investigate the numerical behavior of the quadrature rules for $H=\lambda\in\mathbb{R}$, a scalar.
Second, we consider $H$ to be a matrix and we argue, using two examples, that the results from the scalar case can be used (almost) directly to describe the numerical behavior for the matrix case.

Consider $H = \lambda = 4$ and a shift $z=3.5+0.1i$.
The exact result is $\mathcal{I} = (-0.5+0.1i)^{-1}$ and, for a quadrature rule $\mathcal{I}_K$ with $K$ nodes, we will compute the relative error $\frac{\vert \mathcal{I}-\mathcal{I}_K\vert}{\vert \mathcal{I}\vert}$.
In Figure \ref{fig:scalar_single_epsilon} the three quadrature rules for the single integral are compared for the approximation of $\mathcal{I}$.
For a requested accuracy of $\epsilon=10^{-14}$, the Gauss-Legendre converges fastest, reaching $\mathcal{O}(\epsilon)$ at a cost $t_{\rm tot}\approx 10500$, whereas Gauss-Laguerre requires $t_{\rm tot}\approx 11400$.
Due to its slow rate of convergence, the trapezoidal rule is not competitive.
For $\epsilon=10^{-7}$, see the bottom figure in Figure \ref{fig:scalar_single_epsilon}, the Gauss-Legendre is still the best choice.
Note that a larger $\epsilon$ results in a smaller $T$, which implies a slower oscillating integrand when mapping from $[0,T]$ to $[-1,1]$, where the Gauss-Legendre rule is applied.
A slower oscillating integrand needs fewer quadrature nodes to be resolved, but the maximum accuracy is, naturally, limited to $\epsilon$.
For any choice of $\epsilon$ Gauss-Legendre outperforms the other two quadrature rules.
\begin{figure}[!ht]
    \centering
    \setlength\figureheight{7cm}
    \setlength\figurewidth{0.9\textwidth}	\input{figs/Paper_Scalar_Single_epsilon.tikz}
    \caption{Approximation error for the three quadrature rules for $H=4$, $z=3.5+0.1i$ and requested accuracy $\epsilon=10^{-14}$ in top figure and $\epsilon=10^{-7}$ in bottom figure, marked by dashed green line. Gauss-Legendre ${\color{red} \circ}$, trapezoidal ${\color{blue} \circ}$ and Gauss-Laguerre rule ${\color{black} \ast}$. Top: with respect to number of nodes $K$ and bottom: with respect to total evolution time $t_{\rm tot}$.}
    \label{fig:scalar_single_epsilon}
\end{figure}

In order to get an idea of the cost of computing a resolvent $(z-\lambda)^{-1} = -i\int_0^\infty e^{i(z-\lambda)t}$, we can look at two effects revealed by the integrand $e^{-i(z-\lambda)t} = e^{i(\Re(z)-\lambda)t} e^{-\Im(z)t}$.
The first effect is the decay of the integrand, which is governed by $\Im(z)$, the imaginary part of $z$.
A faster decaying integrand requires fewer quadrature nodes to be resolved, this effect is illustrated in Table \ref{table:scalar_imag_z}, where $H=4$, $\epsilon=10^{-7}$ and $z=3.5+bi$, with $b$ moving closer to the real line.
We see that, as $b$ becomes smaller, the cost of all quadrature rules becomes larger and that the Gauss-Laguerre is more efficient only for larger values of $b$.
Note also that $T$ grows larger with smaller $b$.
\begin{table}[!ht]
\begin{tabular}{l|lllll}
$z$            & $3.5+1i$ & $3.5+0.5i$ & $3.5+0.2i$ & $3.5+0.1i$ & $3.5+0.05i$ \\ \hline
$T$            & 16.811   & 33.622     & 84.056     & 168.11     & 336.22      \\ \hline
Gauss-Legendre & 12       & 13         & 21         & 33         & 55          \\
Trapezoidal    & 21807    & 20541      & 42343      & >50000$^\ast$      &      >50000$^\ast$ \\
Gauss-Laguerre & 8        & 13         & 31         & 62         & 125        
\end{tabular}
\caption{Number of quadrature nodes $K$ required to reach an accuracy of $\epsilon=10^{-7}$ for different $z$ with changing imaginary part $\Im(z)$. For Gauss-Legendre and trapezoidal rule the interval $[0,T]$ is used. $^\ast$The trapezoidal rule is capped at $K=50000$ nodes.}
\label{table:scalar_imag_z}
\end{table}

The second effect is the osccilatory behavior of the integrand, which is governed by $\vert \Re(z)-\lambda\vert$, i.e., the distance of the shift from the eigenvalue.
A larger distance leads to a faster oscillating integrand, and thus, requiring more nodes in the approximation.
In Table \ref{table:scalar_real_z} show the number of nodes needed to reach $\epsilon=10^{-7}$ as the shift $z$ is moved further away from the eigenvalue, with $\Im(z)$ constant.
\begin{table}[]
\begin{tabular}{l|lllll}
$z$            & $2+0.1i$   & $3+0.1i$   & $3+0.1i$ & $3.7+0.1i$ & $4+0.1i$   \\ \hline
Gauss-Legendre & 59         & 34         & 24       & 17         & 34         \\
Trapezoidal    & 1.6713e+05 & 1.1171e+05 & 91574    & 37604      & 1.1171e+05 \\
Gauss-Laguerre & 100        & 62         & 53       & 49         & 62    
\end{tabular}
\caption{Number of quadrature nodes $K$ required to reach an accuracy of $\epsilon=10^{-7}$ for different $z$, changing $\Re(z)$ and constant $\Im(z)$. A larger distance $\vert \Re(z)-\lambda\vert$ leads to a larger number of quadrature nodes needed to reach $\epsilon$.  For Gauss-Legendre and trapezoidal rule the interval $[0,T]$ is used, with $T = 184.21$.}
\label{table:scalar_real_z}
\end{table}

The observations and conclusions for these scalar examples can be straightforwardly applied to any matrix Hermitian $H\in\mathbb{C}^{m\times m}$.
Let $H = XDX^\ast$ denote the eigenvalue decomposition of $H$, with $D$ a diagonal matrix with elements $\{\lambda_j\}_{j=1}^m$.
Then, for some vector $v\in\mathbb{C}^m$, we have $v^\ast e^{iHt}v = v^\ast X e^{iDt}X^\ast v$, which essentially reduces the matrix exponential to a sum of scalar exponentials.
{\color{red} NOTE: remainder of this section must be rewritten.}

\textbf{Subspace example}:
    Consider $H = XDX^\ast$ with a diagonal matrix $D = {\rm diag}(-4,-3,\dots,4) = {\rm diag}(\lambda_1,\lambda_2,\dots,\lambda_9)$ and a unitary matrix $X = \begin{bmatrix}
        x_1 & x_2 & \cdots x_{9}
    \end{bmatrix}$.
    We are interested in approximating the resolvent applied to a vector $v$, i.e., $(z-H)^{-1} v$.
    The approximation consists of evaluations of the matrix exponential $e^{i(z-H)t}$.

    Let $X = I = \begin{bmatrix}
        e_1 & e_2 & \dots & e_{9}
    \end{bmatrix}$, and we consider three different vectors, $v_1 = \frac{1}{\sqrt{2}}(e_1 + e_{9})$, $v_2 = e_{9}$ and $v_3 = \frac{1}{\sqrt{2}}(e_5 + e_{9})$.
    We fix $z = 3.5+1i$ and will approximate $(z-H)^{-1} v_k$.
     
    For different choices of $v$, the approximation error is shown in Figure \ref{fig:matvec_v2}.
    Clearly, the convergence for $v_2$ is much faster. This can be explained by looking at the eigenvalues that are excited by the vector.
    Since, $e^{i(z-H)t} = e^{i(a-H)t} e^{-bt}$, the highest oscillation in $e^{i(a-H)t}$ is $\alpha = \underset{n}{\max} \vert a-\lambda_n\vert$.
    When computing $e^{i(z-H)t} v$, the eigenvalues that are excited are those corresponding to the eigenvectors present in $v$.
    Thus, for $v_1$ we have $\alpha_1 = \max(\vert a-\lambda_1 \vert,\vert a-\lambda_9 \vert) = 7.5$ and for $v_2$, we have $\alpha_2 = \vert a-\lambda_9\vert = 0.5$, explaining the difference in convergence since higher oscillatory integrands require more nodes for the quadrature rule.
    For $v=v_3$, and since $\alpha = 3.5$, we get a convergence rate that is slower than $v_2$ and faster than $v_1$.
    \begin{figure}[!ht]
	\centering
	\setlength\figureheight{12cm}
	\setlength\figurewidth{0.9\textwidth}
	\input{figs/SubspaceExperiment.tikz}
	\caption{Approximation error for $(z-H)^{-1}v$, for $H=D$, $z=3.5+1i$. Top: $v=v_1$ , middle: $v=v_2$ ,and bottom: $v=v_3$. Gauss-Legendre {\color{red}$\circ$}, Trapezoidal {\color{blue}??}, and Gauss-Laguerre {\color{black} $\ast$}.} 
	\label{fig:matvec}
    \end{figure}
    
    \textbf{Remark:} Without loss of generality we could take $X=I$ in our experiments, since, for any matrix in its eigenvalue decomposition $H = XDX^{-1}$, we have $e^{i(z-H)t} = X e^{i(z-D)t}X^{-1}$.

    In general the decomposition of a vector $v$ in terms of the eigenvector of $H$ is unknown, hence, we cannot determine $\alpha$ by maximization restricted to the invariant subspace.
    The use of $\alpha$ maximized over all eigenvalues can, as shown above, provide a large overestimation of the required number of nodes for the quadrature rules.
    In contour integration, we can get a better upper bound on $\alpha$, See Section \ref{sec:contour_experiments}.

    \subsubsection{Numerical experiments -- double integral}
    

    \subsubsection{Contour integration}\label{sec:contour_experiments}
    In the context of contour integration, we are only interested in a subdomain of the spectrum of $H$, that is, those eigenvalues lying in a given interval $[J_1,J_2]$.
    A contour $\Omega$ in the complex plane is chosen which encircles this interval and crosses the real line at $J_1$ and $J_2$, e.g., the circle centered at $c = \frac{J_1+J_2}{2}$ and radius $r = \frac{J_2-J_1}{2}$.
    Then, the endpoints of the interval can be used to get an upper bound on $\alpha$ in the invariant subspace spanned by the eigenvectors of eigenvalues in the interval $[J_1,J_2]$, i.e., $\alpha < \underset{n}{\max} \{ \vert \Re z-J_1\vert,\vert \Re z-J_2\vert \}$.

    We illustrate this with the following example.
    Consider $H = XDX^\ast$, with $D = {\rm diag}([-10,-0.3,0,1,10])$ and $X = \begin{bmatrix} x_1 &  x_2 & x_3 & x_4 & x_5\end{bmatrix}$ a random unitary matrix.
    Suppose we are interested in the action of the matrix exponential $e^H$, but only on its effect on eigenvalues in the interval $[-2,2]$, which can be written as a contour integral
    \begin{equation*}
        I_\Gamma := \frac{1}{2\pi i}\oint_\Gamma e^z (z-H)^{-1} dz,
    \end{equation*}
    where $\Gamma$ encircles the interval.
    Thus, $I_\Gamma$ approximates $S^\ast e^H S$, where $S = \begin{bmatrix} 0 &  x_2 & x_3 & x_4 & 0\end{bmatrix}$, note that we do not need to know these eigenvectors, they are only used to facilitate the discussion.
    
    Take $\Gamma = \{2e^{i\theta}\vert \theta\in[0,2\pi]\}$, and use the $N$-node trapezoidal rule to discretize the integral
    \begin{equation*}
        I_\Gamma = \frac{1}{\pi }\int_{0}^{2\pi} e^{2e^{i\theta}} (2e^{i\theta}-H)^{-1} e^{i\theta}d\theta  \approx h/\pi \sum_{k=1}^N e^{2e^{i\theta_k}} e^{i\theta_k} (2e^{i\theta_k}-H)^{-1}=: I_{\Gamma,N},
    \end{equation*}
    with $h = \frac{2\pi}{N}$ and $\theta_k = kh$, $k=1,2,\dots, N$.

    The resolvents $(2e^{i\theta_k}-H)^{-1}$ required in the quadrature rule are approximated by $\mathcal{I}_N$ {\color{red}as described in Section \ref{}}, the resulting approximation of $I_{\Gamma,N}$ is denoted by $I_{\Gamma,N}^Q$, where $Q$ refers to the fact that the resolvents are approximated using quadrature rules.
    These resolvents are computed up to precision $\epsilon$ measured in the subspace spanned by $S$, i.e., ${\rm err}_S := \frac{\Vert S^\ast (2e^{i\theta_k}-H)^{-1}S -  \mathcal{I}_N \Vert_2}{\Vert S^\ast(2e^{i\theta_k}-H)^{-1}S \Vert_2}\leq \epsilon$.
    The error ${\rm err} := \frac{\Vert (2e^{i\theta_k}-H)^{-1} -  \mathcal{I}_N \Vert_2}{\Vert (2e^{i\theta_k}-H)^{-1} \Vert_2}$ is tracked as well.
    
    For each node $\theta_k$ the resolvent is approximated such that ${\rm err}_S \leq \epsilon = 10^{-8}$. 
    We observe that ${\rm err} \approx \mathcal{O}(10^{-1})$ for all $\theta_k$.
    The approximation error ${\rm err}_N:=\frac{\Vert S^\ast e^H S- I_{\Gamma,N}\Vert_2}{\Vert S^\ast e^H S\Vert_2} $ using exact resolvents, and the approxmation error ${\rm err}_N^Q:=\frac{\Vert S^\ast e^H S- I_{\Gamma,N}^Q\Vert_2}{\Vert S^\ast e^H S\Vert_2} $, using approximations to the resolvents, are shown in Figure \ref{fig:contour_expm}.
    We see that these errors are equal until the accuracy $\epsilon=10^{-8}$ is reached and, since the approximated resolvent are only accurate up to $\epsilon$, the error ${\rm err}_N^Q$ stagnates at around $\mathcal{O}(\epsilon)$.
    On the other hand, ${\rm err}_N^Q$ reaching the accuracy $\mathcal{O}(\epsilon)$ verifies that the resolvent approximation only has to be accurate for the eigenvalues of interest, i.e., it corresponds to the error on the subspace ${\rm err}_S $ and not to the much larger error measured on the whole space ${\rm err}$.
    If $\epsilon$ is chosen larger, e.g., $\epsilon = 10^{-4}$, then the highest attainable accuracy for the contour integration changes accordingly.
    \begin{figure}[!ht]
	\centering
	\setlength\figureheight{5cm}
	\setlength\figurewidth{0.9\textwidth}
	\input{figs/contour_expm.tikz}
	\caption{Approximation of $e^H$ by contour integration and trapezoidal rule, using exact resolvents ${\rm err}_N:=\frac{\Vert S^\ast e^H S- I_{\Gamma,N}\Vert_2}{\Vert S^\ast e^H S\Vert_2}$ ({\color{blue}$\ast$}), and approximating the resolvents with real time evolution $\frac{\Vert S^\ast e^H S- I_{\Gamma,N}^Q\Vert_2}{\Vert S^\ast e^H S\Vert_2}$ up to $\epsilon=10^{-8}$ in ({\color{red}$\circ$}) and up to $\epsilon=10^{-4}$ in ({\color{green}$+$}) .}
	\label{fig:contour_expm}
    \end{figure}

    
    This experiment shows that it is indeed appropriate to upper bound $\alpha < \underset{n}{\max} \{ \vert \Re z-J_1\vert,\vert \Re z-J_2\vert \}$, which quantifies the cost.



\subsection{Trotterization}
Let $H$ be a Hamiltonian that can be written as a sum $H =\sum_j H_j$, where each term allows for an efficient real time evolution, i.e., efficient computation of $e^{-iH_j t}$.
Then, for a finite number $N$ and corresponding step size $\Delta t = t/N$, the first order Trotter method is
\begin{equation*}
    e^{-iHt} \approx \left(\prod_j e^{iH_j \Delta t}\right)^N,
\end{equation*}
which has an error $\mathcal{O}(\Delta t^2 N)$ {\color{red} TODO: this holds for 2 terms, what is the error for more terms?}.
In order to reach precision $\delta$, take $N = \mathcal{O}(t^2 \delta^{-1})$.

For equidistant nodes, e.g., in the trapezoidal rule,  a fixed time step size $\Delta t$ can be used directly.
For the nodes of Gauss-Legendre and Gauss-Laguerre, the distance between the nodes is not constant.
A fixed time step $\Delta t$ is used to approach the node $t_k$ of interest, let us say that $N$ steps are required such that $t_k-N \Delta t <\Delta t$ holds, and a single smaller time step $\tau := t_k-N \Delta t$ provides us with the appropriate approximation.
That is, for $t_k = N\Delta t + \tau$, with $\tau<\Delta t$, we use
\begin{equation*}
        S(H, t_k, \Delta t) := \left(\prod_j e^{iH_j \Delta t}\right)^N \prod_j e^{iH_j \tau}.
    \end{equation*}

\textbf{TFIM}
In the transverse field Ising model (TFIM), the Hamiltonian is given by 
\begin{equation*}
     H =  -J \underset{\langle i,j\rangle}{\sum} Z_i Z_j - g\underset{j}{\sum} X_j,
\end{equation*}
with spin-spin coupling $J$ and transverse field $g$.
For Trotterization $H$ is split up into $H = H_1+H_2$,
\begin{equation*}
    H_1 = -J  \underset{\langle i,j\rangle}{\sum} Z_i Z_j, \qquad H_2 = - g\underset{j}{\sum} X_j.
\end{equation*}


\textbf{Pauli string}
\begin{figure}[!ht]
	\centering
	\setlength\figureheight{5cm}
	\setlength\figurewidth{0.9\textwidth}
	\input{figs/Trotter_Pauli_n=6_l=20_seed=45.tikz}
	\caption{Effect of Trotterization on the }
	\label{fig:Trotter_Pauli}
    \end{figure}


